Logic Query of Thoughts: Guiding Large Language Models to Answer Complex Logic Queries with Knowledge Graphs

Despite the superb performance in many tasks, large language models (LLMs) bear the risk of generating hallucination or even wrong answers when confronted with tasks that demand the accuracy of knowledge. The issue becomes even more noticeable when addressing logic queries that require multiple logic reasoning steps. On the other hand, knowledge graph (KG) based question answering methods are capable of accurately identifying the correct answers with the help of knowledge graph, yet its accuracy could quickly deteriorate when the knowledge graph itself is sparse and incomplete. It remains a critical challenge on how to integrate knowledge graph reasoning with LLMs in a mutually beneficial way so as to mitigate both the hallucination problem of LLMs as well as the incompleteness issue of knowledge graphs. In this paper, we propose 'Logic-Query-of-Thoughts' (LGOT) which is the first of its kind to combine LLMs with knowledge graph based logic query reasoning. LGOT seamlessly combines knowledge graph reasoning and LLMs, effectively breaking down complex logic queries into easy to answer subquestions. Through the utilization of both knowledge graph reasoning and LLMs, it successfully derives answers for each subquestion. By aggregating these results and selecting the highest quality candidate answers for each step, LGOT achieves accurate results to complex questions. Our experimental findings demonstrate substantial performance enhancements, with up to 20% improvement over ChatGPT.

==> 010equipment_require.tex <==


The system runs on a moderate desktop with an Intel Core-i7 3.00GHz CPU and 64GB memory. The operation system is win10.
The front-end of the system is implemented by HTML, Javascript and D3.js.
The back-end of the system is implemented by Flask, python, redis and C++. 
The Web platform based design provides a natural way to interact with the audience in the virtual environment through a web browser. No special equipment is needed for the audience. We will provide a short video to provide step-by-step instructions on how users can interact with the system in the virtual environment.

We will run live demonstrations and allow for open interactions with the audience. This includes the ability for audience members to run various queries and explore the reasoning results. Our goal is to spark a healthy discussion on knowledge graph reasoning in terms of the algorithmic and systemic challenges, as well as the potential applications and future directions. 
%To run the system, users need to install Flask, redis, python and C++ package, then start the system.
